Learning with Noisy Labels by Efficient Transition Matrix Estimation to Combat Label Miscorrection

Recent studies on learning with noisy labels have shown remarkable performance by exploiting a small clean dataset. In particular, model agnostic meta-learning-based label correction methods further improve performance by correcting noisy labels on the fly. However, there is no safeguard on the label miscorrection, resulting in unavoidable performance degradation. Moreover, every training step requires at least three back-propagations, significantly slowing down the training speed. To mitigate these issues, we propose a robust and efficient method that learns a label transition matrix on the fly. Employing the transition matrix makes the classifier skeptical about all the corrected samples, which alleviates the miscorrection issue. We also introduce a two-head architecture to efficiently estimate the label transition matrix every iteration within a single back-propagation, so that the estimated matrix closely follows the shifting noise distribution induced by label correction. Extensive experiments demonstrate that our approach shows the best performance in training efficiency while having comparable or better accuracy than existing methods.

==> Figures/4_5_Label_Correction.tex <==
\begin{figure*}[t]
% \begin{wrapfigure}{R}{0.35\textwidth}
\begin{minipage}{0.49\textwidth}
% \vspace{-3.5em}
% \begin{figure}[t] %%% t: top, b: bottom, h: here
\centering
\includegraphics[width=\linewidth]{figures/label_correction_effect_plot.pdf}

\caption{
Effect of label correction on CIFAR-10/100 with various symmetric noise ratio. Accuracy (\%) of FasTEN (ours.) and FasTEN without label correction is provided.
}
% \vspace{-3em}
\label{fig:relabel}
% \end{figure}
\end{minipage}
\hfill
\begin{minipage}{0.49\textwidth}
% \vspace{-3.5em}
% \begin{figure}[t] %%% t: top, b: bottom, h: here

\centering
\includegraphics[width=1.0\linewidth]{figures/label_correction_threshold_plot.pdf}

% \vspace{-0.2cm}
\caption{
Robustness to Mis-labeling of FasTEN. 
The corrected label amount (\%) and model accuracy (\%) according to the label correction threshold ($\rho$) are provided.
% Effect of label correction on CIFAR-10/100 with various symmetric noise ratio.
% Accuracy (\%) of \textbf{FasTEN (ours.)} and FasTEN without label correction is provided.
}
\label{fig:relabel_amount}
% \end{figure}
\end{minipage}
% \end{wrapfigure}
\end{figure*}


==> Figures/4_Robustness_to_Miscorrected_Labels.tex <==
\begin{figure}[h]
% \begin{wrapfigure}{R}{0.35\textwidth}
% \vspace{-3.5em}
% \begin{figure}[t] %%% t: top, b: bottom, h: here
\centering
\includegraphics[width=0.65\linewidth]{Figures/4_Robustness_to_Miscorrected_Labels_Plot.pdf}
\caption{
Robustness to miscorrected labels on CIFAR-10 with various perturbation strength. Test accuracy (\%) of baselines and baselines without the label correction is provided.
}
\label{fig:safeguard}
\end{figure}


==> Figures/5_Transition_Matrix.tex <==
\begin{figure}[h]
% \begin{wrapfigure}{R}{0.35\textwidth}
% \vspace{-3.5em}
% \begin{figure}[t] %%% t: top, b: bottom, h: here
\centering
\includegraphics[width=0.9\linewidth]{Figures/5_Transition_Matrix_Plot.pdf}
\caption{
The plot for the mean of the diagonal term in oracle transition matrix $T$ and our estimated transition matrix $\widehat{T}$ according to the epoch on CIFAR-10 dataset with asymmetric 40\% and symmetric 80\% noise.}
% \vspace{-3em}
\label{fig:transition_matrix}
\end{figure}


==> Figures/7_Safeguard.tex <==
\begin{figure}[h]
% \begin{wrapfigure}{R}{0.35\textwidth}
% \vspace{-3.5em}
% \begin{figure}[t] %%% t: top, b: bottom, h: here
\centering
\includegraphics[width=0.65\linewidth]{Figures/7_Safeguard_Plot.pdf}
\caption{
\textcolor{red}{Robustness to miscorrected labels on CIFAR-10 with various perturbation strength. Test accuracy (\%) of baselines and baselines without the label correction is provided. HAVE TO DELETE THIS.}
}
% \vspace{-3em}
\label{fig:safeguard}
\end{figure}

